Anonimos: An LP based Approach for Anonymizing Weighted Social Network Graphs

The increasing popularity of social networks has initiated a fertile research area in information extraction and data mining. Anonymization of these social graphs is important to facilitate publishing these data sets for analysis by external entities. Prior work has concentrated mostly on node identity anonymization and structural anonymization. But with the growing interest in analyzing social networks as a weighted network, edge weight anonymization is also gaining importance. We present An\'onimos, a Linear Programming based technique for anonymization of edge weights that preserves linear properties of graphs. Such properties form the foundation of many important graph-theoretic algorithms such as shortest paths problem, k-nearest neighbors, minimum cost spanning tree, and maximizing information spread. As a proof of concept, we apply An\'onimos to the shortest paths problem and its extensions, prove the correctness, analyze complexity, and experimentally evaluate it using real social network data sets. Our experiments demonstrate that An\'onimos anonymizes the weights, improves k-anonymity of the weights, and also scrambles the relative ordering of the edges sorted by weights, thereby providing robust and effective anonymization of the sensitive edge-weights. Additionally, we demonstrate the composability of different models generated using An\'onimos, a property that allows a single anonymized graph to preserve multiple linear properties.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Anonymization of edge weights in a social network graph is important for enabling the analysis and mining of social graphs by computer scientists as well as social scientists. Such mining has significant impact on the management of social networks as well as the understanding of various social behaviors. We proposed \anonimos, a technique for the effective anonymization of weighted social network graphs by modeling \emph{linear properties} and formulating them as an LP problem. The \anonimos\ approach is fairly straightforward and can be applied to preserve any \emph{linear property} by a simple generation of inequalities corresponding to decisions made by the algorithm during its execution. As a proof of concept, we considered the \emph{shortest paths problem} and showed how off-the-shelf LP packages can be used to effectively anonymize the graphs. The \emph{composability} of \anonimos\ for preserving multiple properties in a single anonymized graph was demonstrated using the \emph{all pairs shortest paths} problem. We also showed how a careful analysis of the properties can result in significant reductions in complexity of the models. Our experiments demonstrated the effectiveness of our techniques in the anonymization of graphs, and the efficacy of our optimizations, while ensuring that the desired properties are preserved across anonymization. In the future, we would like to explore extensions of \anonimos\ for other applications such as graph clustering, information spread modeling, etc., which also rely on linear combinations of edge weights.

\section*{Acknowledgement}

The authors would like to thank Divyakant Agrawal, Pamela Bhattacharya, and Sayan Ranu for their insightful comments on the earlier versions of the paper which has helped in improving this paper. The authors would also like to thanks Alan Mislove for providing the data sets used for the experiments. This work is partially supported by NSF Grants IIS-0744539 and IIS-0847925.


==> related.tex <==
\section{Related work}
\label{sec:related}

The need to protect the privacy of social entities involved in social networks has given rise to
active research in anonymization techniques for social network graphs.
This interest has been primarily driven by the findings of
Backstrom et~al.~\cite{backstrom07} and Korolova et~al.~\cite{korolova08}. Backstrom et al.~\cite{backstrom07} described a technique based on the structural properties of graphs such as isomorphism
and automorphism to re-identify vertices in the anonymized graph. Their technique was based on implanting unique structures in the graph which can be re-identified in the anonymized graph  with very high probability. On the other hand, Korolova et~al.~\cite{korolova08} devised an attack where a node can be re-identified based in part on background information regarding the neighborhood. As a result, a lot of research has focused on \emph{node identity anonymization} and \emph{structural anonymization}. A comprehensive survey about the various anonymization techniques is provided in~\cite{liu08book,wu10_book}.


A class of proposals, by Hay et~al.~\cite{hay08}, Zhou et~al.~\cite{zhou07}, Liu et~al.~\cite{liu08}, and Zou et~al.~\cite{zou09_kautomorphism}, suggest different methods for anonym\-ization that are based on the addition and/or deletion of edges in the graph for altering the structure of the graph and the prevention of re-identification in the anonymized graph. On the other hand, Cormode et~al.~\cite{cormode08c} suggest a technique for the anonymization of bipartite graphs based on safe groupings, an extension of which is class based anonymization~\cite{cormode_vldb09_class}. Ying et~al.~\cite{ying08} propose a randomization based spectrum preserving approach which effectively preserves the properties of the eigenvalues of the network, while anonymizing the edges, and Campan et~al.~\cite{campan08} suggest a clustering based approach for node anonymization. Along different lines, Zheleva et~al.~\cite{zheleva07} formulate the problem of edge re-identification in an unweighted graph, where the edge labels are sensitive.% and need to be anonymized.

The majority of existing work considers unweighted graphs for node identity and structural
anonymization. But as reflected by recent work~\cite{kumpula07,toivonen07}, the weighted social network
model is gaining importance, and so is edge weight anonymization.
Liu et~al.~\cite{liu09sdm} suggest a probabilistic technique for
anonymizing edge weights by perturbing the actual edge weights by a small $\sigma$ obtained from
a probability distribution. The goal is to keep the total
cost of the shortest path close to the cost of the path in the original graph.
However in this approach, the anonymized weights are
close to the original edge weights, and hence may reveal
sensitive information about the original values.
\anonimos\ aims at preserving general linear properties of the
graph. For the shortest paths, our goal is to preserve the paths rather than
the values and for most applications, the ability to reconstruct the
actual path is more important than maintaining approximate values.
In addition, if necessary, our model can approximately preserve the cost of the shortest paths as well
by adding constraints of the form $f(u,\ldots,v) = D[u,v] \pm \epsilon$. Note that since the edge weights are only perturbed by a small value, the technique of~\cite{liu09sdm} can neither significantly improve \emph{k-anonymity}, nor can it scramble the ordering of edge weights.


